Learning Morphisms with Gauss-Newton Approximation for Growing Networks

A popular method for Neural Architecture Search (NAS) is based on growing networks via small local changes to the network's architecture called network morphisms. These methods start with a small seed network and progressively grow the network by adding new neurons in an automated way. However, it remains a challenge to efficiently determine which parts of the network are best to grow. Here we propose a NAS method for growing a network by using a Gauss-Newton approximation of the loss function to efficiently learn and evaluate candidate network morphisms. We compare our method with state of the art NAS methods for CIFAR-10 and CIFAR-100 classification tasks, and conclude our method learns similar quality or better architectures at a smaller computational cost.

==> fig/experiments-figures.tex <==
\begin{figure*}[h]
\centering
\subfigure[]{
    \includegraphics[scale=0.35]{fig/fig-gn-approx/epoch-40/layer0.pdf}
    \label{fig:gn-approx-epoch-40-layer0}
}
\hfill
\subfigure[]{
    \includegraphics[scale=0.35]{fig/fig-gn-approx/epoch-40/layer8.pdf}
    \label{fig:gn-approx-epoch-40-layer8}
}
\hfill
\subfigure[]{
    \includegraphics[scale=0.35]{fig/fig-gn-approx/epoch-40/layer15.pdf}
    \label{fig:gn-approx-epoch-40-layer15}
}
\caption{Estimated versus actual decrease in loss for morphisms learned while holding model parameters constant. }
\label{fig:gn-approx-epoch-40}
\end{figure*}

\begin{figure*}[h]
\centering
\includegraphics[scale=0.8]{fig/compare-directions-no-title.pdf}
\caption{Comparison of different morphism learning strategies. Each $3$-bar cluster plots the true decrease in loss achieved by the channel-splitting morphism learned by each method for one of the $64$ channels in the first layer of VGG-19. }
\label{fig:compare-directions}
\end{figure*}

==> tex/gauss-newton.tex <==
In this section we review the justification for Gauss-Newton approximation. We begin by assuming that the loss function is well-approximated by a least-squares problem in $z$, i.e., for some matrix $A$ and vector $b$,
\begin{align*}
\mathcal L(z) &\approx \frac{1}{2} \| Az - b \|_2^2 \\
&= \frac{1}{2} b^\top b - z^\top A^\top b + \frac{1}{2} z A^\top A z.
\end{align*}
Denote the residual:
\begin{align*}
    r = Az - b
\end{align*}
Note that $\mathcal L = \frac{1}{2} r^\top r$. Denote the gradient and Hessian of the loss:
\begin{align*}
    g &= A^\top r & H &= A^\top A
\end{align*} Consider the change in the loss function when adding a quantity $\Delta z$ to $z$. Denote the change in loss:
\begin{align*}
\Delta \mathcal L(\Delta z) &\equiv \mathcal L(z + \Delta z) - \mathcal L(z) \\
&= \Delta z \cdot g + \frac{1}{2} \Delta z^\top A^\top A \Delta z \\
&= \Delta z \cdot g + \frac{1}{2} \Delta z^\top H \Delta z \\
\end{align*}
In this paper, we write the Gauss-Newton approximation as
\[
H \approx \frac{1}{2 \mathcal L} g g^\top,
\]
\begin{theorem}[General Gauss-Newton Approximation]
If ${\Delta z = \lambda \Delta z^*}$ for some $\lambda \in \mathbb R$ and some $\Delta z^*$ satisfying $A (z + \Delta z^*) = b$, then
\[
\frac{1}{2} \Delta z^\top H \Delta z = \frac{1}{2} \Delta z \frac{gg^\top}{2 \mathcal L} \Delta z
\]
\end{theorem}
\begin{proof}
If ${\Delta z = \lambda \Delta z^*}$ and $A (z + \Delta z^*) = b$, then ${A \Delta z = - \lambda r}$. So
\begin{gather*}
 \frac{1}{2} \Delta z^\top \left( \frac{g g^\top}{2 \mathcal L} \right) \Delta z \\
= \frac{1}{2} \Delta z^\top \left( \frac{A^\top r r^\top A}{r^\top r} \right) \Delta z \\
= \frac{1}{2} \lambda^2 r^\top r
\end{gather*}
Similarly,
\begin{align*}
    \frac{1}{2} \Delta z^\top H  \Delta z &= \frac{1}{2} \Delta z A^\top A \Delta z \\
    &= \frac{1}{2} \lambda^2 r^\top r
\end{align*}
\end{proof}
Therefore, we say the Gauss-Newton approximation is exact in the space spanned by the solutions $\Delta z^*$ to the linear system $A (z + \Delta z^*) = b$.
\begin{theorem} [Rank-1 Gauss-Newton Approximation]
If $H$ is rank-1 and there exists a solution $z^*$ to the linear system $A z^* = b$, then for all $\Delta z$,
\[
\frac{1}{2} \Delta z^\top H \Delta z = \frac{1}{2} \Delta z \frac{gg^\top}{2 \mathcal L} \Delta z
\]
\end{theorem}
\begin{proof}
If $H$ is rank-1, then $A$ consists of a single row $u^\top$ and $b \in \mathbb R$ is a scalar.

Let $\Delta z$ be arbitrary. Then there exists a solution $\Delta z^*$ to the linear system $A(z + \Delta z^*) = b$ and $\lambda \in \mathbb R$ such that $\Delta z = \lambda \Delta z^*$, namely
\begin{gather*}
     \Delta z^* = \frac{b - u^\top z}{u^\top z} \Delta z \\
     \lambda = \frac{u^\top \Delta z}{b - u^\top z}
\end{gather*}
since then
\begin{align*}
    A(z + \Delta z^*) &= u^\top z + u^\top \Delta z^* \\
    &= u^\top z + u^\top \left( \frac{b - u^\top z}{u^\top z} \Delta z \right) \\
    &= b
\end{align*}
Applying the previous theorem yields the result.
\end{proof}
From this it is clear that we can expect the Gauss-Newton approximation to be quite accurate if the true Hessian matrix $H$ is low-rank.

==> tex/results-tables.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Method Type & Reference & Error (\%) & Params & Reachable? & GPU time \\
 &  & & (Millions) & & (days) \\
\hline \hline
\multirow{3}{*}{SOTA} 
& AmoebaNet-A \cite{real2019regularized}      & 3.3 &  3.2 &  & $3150$ \\
& NASNET-A \cite{zoph2018learning}            & 3.4 &  3.3 &  & $2000$ \\
& Large-scale Evolution \cite{real2017large}  & 5.4 &  5.4 &  & $2600$ \\
\hline \hline
\multirow{4}{*}{Morphisms} 
& NASH \cite{elsken2017simple}                                  & 5.2 & 19.7 & \checkmark & $1.0$ \\
& Slimming \cite{liu2017learning} & 6.2 & 2.3 & \checkmark & - \\& Firefly \cite{wu2020firefly}                                 & 6.2 &  1.9 & \checkmark & - \\
& Net2Net \cite{chen2015net2net}                                 & 6.5 &  3.9 & \checkmark & $2.1$ \\
\hline \hline
\multirow{4}{*}{Human-\newline Designed} 
& DenseNet \cite{huang2017densely}                              & 3.5 & 25.6 &  & N/A \\
& VGG-19 Baseline \cite{simonyan2014very}                          & 6.3 & 20.0 & \checkmark & N/A \\
& ResNet \cite{huang2016deep}                                      & 6.4 &  1.7 &  & N/A \\
& MobileNetV1 Baseline \cite{howard2017mobilenets}                 & 6.6 & 3.2 & \checkmark & N/A \\
\hline \hline
\multirow{5}{*}{Ours} 
& Seed VGG-19, $\lambda_p = 3 \times 10^{-7}$         & 5.6 & 1.2 & \checkmark & $0.7$ \\
& Seed VGG-19, $\lambda_p = 1 \times 10^{-6}$        & 6.5 & 0.6 & \checkmark & $0.5$ \\
& Seed MobileNetV1, $\lambda_p = 3 \times 10^{-8}$ & 5.8 & 0.8 & \checkmark & $1.0$ \\
& Seed MobileNetV1, $\lambda_p = 3 \times 10^{-7}$ & 6.0 & 0.5 & \checkmark & $1.0$ \\
& Seed MobileNetV1, $\lambda_p = 1 \times 10^{-6}$ & 6.2 & 0.4 & \checkmark & $0.7$ \\
\hline
\end{tabular}
\caption{Classification performance of various architectures on CIFAR-10}
\label{table:cifar10}
\end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Method Type & Reference & Error (\%) & Params & Reachable? & GPU time \\
 &  & & (Millions) & & (days) \\
\hline \hline 
\multirow{2}{*}{SOTA}
& Large-scale Evolution \cite{real2017large}  & 23.0 & 40.4 &  & - \\
& SMASH \cite{brock2017smash} & 22.1 & 4.6 &  & - \\
\hline \hline
\multirow{2}{*}{Morphisms}
& NASH \cite{elsken2017simple}  & 23.4 & 22.3 & \checkmark & $1.0$ \\
& Slimming \cite{liu2017learning} & 26.5 & 5.0 & \checkmark & - \\
\hline \hline
\multirow{4}{*}{Human-Designed}
& DenseNet \cite{huang2017densely}        & 17.2 & 25.6 & & N/A \\
& Resnet \cite{he2016deep}                & 27.2 & 1.7 & & N/A \\
& VGG-19 Baseline \cite{simonyan2014very}                         & 27.6 & 20.1 & \checkmark & N/A \\
& MobileNetV1 Baseline \cite{howard2017mobilenets}                   & 28.7 & 3.3 & \checkmark & N/A \\
\hline \hline
\multirow{5}{*}{Ours} 
%& Seed VGG-19 $\lambda_p = 1 \times 10^{-6}$ & 27.9 & 1.6 & \checkmark & ? \\
%& Seed VGG-19, $\lambda_p = 1 \times 10^{-7}$ & 25.6 & 42.6 & \checkmark & ? \\
%& Seed VGG-19, $\lambda_p = 1 \times 10^{-6}$ & 26.4 & 6.6 & \checkmark & ? \\
%& Seed VGG-19, $\lambda_p = 6 \times 10^{-7}$ & 28.3 & 4.9 & \checkmark & ? \\
& Seed VGG-19, $\lambda_p = 3 \times 10^{-7}$ & 27.2 & 2.2 & \checkmark & 0.7 \\
& Seed VGG-19, $\lambda_p = 6 \times 10^{-7}$ & 28.0 & 1.6 & \checkmark & 0.6 \\
& Seed MobileNetV1, $\lambda_p = 1 \times 10^{-6}$ & 27.2 & 0.8 & \checkmark & 0.8 \\
& Seed MobileNetV1, $\lambda_p = 6 \times 10^{-7}$ & 26.9 & 1.3 & \checkmark & 1.0 \\
& Seed MobileNetV1, $\lambda_p = 3 \times 10^{-7}$ & 25.9 & 1.4 & \checkmark & 1.0 \\
\hline
\end{tabular}
\caption{Classification performance of various architectures on CIFAR-100}
\label{table:cifar100}
\end{table*}
